Searches For The Standard Model Higgs Boson in final states with tau leptons at the Tevatron

We present the status of the Standard Model Higgs boson searches in final states containing {\tau} leptons using data collected from p-pbar collisions at Fermilab Tevatron collider at center-of-mass energy of 1.96 TeV. A summary of the latest results from CDF and D0 collaborations is reported in this paper.

==> dpf2011_template_abstrac.tex <==
We present the status of the Standard Model Higgs boson searches in final states containing $\tau$ leptons using data collected
from $p\bar{p}$ collisions at Fermilab Tevatron collider at $\sqrt{s}= 1.96 \ \TeV$. A summary of the latest
results from CDF and D0 collaborations is reported in this paper.
